Search for ttbar resonances in the lepton plus jets final state in ppbar collisions at sqrt{s}=1.96TeV

We present a search for a narrow-width heavy resonance decaying into top quark pairs X->ttbar in ppbar collisions at sqrt{s}=1.96TeV using approximately 0.9fb^-1 of data collected with the D0 detector at the Fermilab Tevatron Collider. This analysis considers ttbar candidate events in the lepton plus jets channel with at least one identified b jet and uses the ttbar invariant mass distribution to search for evidence of resonant production. We find no evidence for a narrow resonance X decaying to ttbar. Therefore, we set upper limits on sigma*B(X->ttbar) for different hypothesized resonance masses using a Bayesian approach. For a Topcolor-assisted technicolor model, the existence of a leptophobic Z' boson with mass M_Z'<700GeV and width Gamma_Z'=0.012 M_Z' can be excluded at the 95% C.L.

==> list_of_visitor_addresses_r2.tex <==
% list_of_visitor_addresses_r2.tex                         3/27/08
%  available symbols are:
%  $\ast, \dag, \ddag, \S, \P, $\|$, $\ast\ast$, \dag\dag, \ddag\ddag ,\#
%
\bibitem[a]{alton}
Visitor from Augustana College, Sioux Falls, SD, USA.
\bibitem[b]{burdin}
Visitor from The University of Liverpool, Liverpool, UK.
\bibitem[c]{podesta-lerma}
Visitor from ICN-UNAM, Mexico City, Mexico.
\bibitem[d]{quadt,meyer,hensel,park}
Visitor from II. Physikalisches Institut, Georg-August-University, G{\"o}ttingen, Germany.
\bibitem[e]{voutilainen}
Visitor from Helsinki Institute of Physics, Helsinki, Finland.
\bibitem[f]{wenger}
Visitor from Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland.
%\bibitem[?]{coadou}
%Visitor from Simon Fraser University, Vancouver, B.C., Canada.
%\bibitem[?]{kozminski}
%Visitor from Lewis University, Romeoville, IL, USA.
\bibitem[\ddag]{deceased}
Deceased.

%
\vskip 0.25cm

